Deficiency-Aware Masked Transformer for Video Inpainting

Recent video inpainting methods have made remarkable progress by utilizing explicit guidance, such as optical flow, to propagate cross-frame pixels. However, there are cases where cross-frame recurrence of the masked video is not available, resulting in a deficiency. In such situation, instead of borrowing pixels from other frames, the focus of the model shifts towards addressing the inverse problem. In this paper, we introduce a dual-modality-compatible inpainting framework called Deficiency-aware Masked Transformer (DMT), which offers three key advantages. Firstly, we pretrain a image inpainting model DMT_img serve as a prior for distilling the video model DMT_vid, thereby benefiting the hallucination of deficiency cases. Secondly, the self-attention module selectively incorporates spatiotemporal tokens to accelerate inference and remove noise signals. Thirdly, a simple yet effective Receptive Field Contextualizer is integrated into DMT, further improving performance. Extensive experiments conducted on YouTube-VOS and DAVIS datasets demonstrate that DMT_vid significantly outperforms previous solutions. The code and video demonstrations can be found at github.com/yeates/DMT.

==> supp_fig/supp_teaser.tex <==


\centering \centering
\begin{overpic}[width=\textwidth]{supp_fig/more_vi_compare.pdf}
\small
\put(3.7,-1.5){Masked Frames}
\put(24,-1.5){FuseFormer~\cite{liu21fuseformer}}
\put(45,-1.5){E$^2$FGVI~\cite{li22e2fgvi}}
\put(66,-1.5){FGT~\cite{zhang22flow}}
\put(86.8,-1.5){Ours}
\end{overpic}
\vspace{0.5mm}
\captionsetup[figure]{aboveskip=0.1cm}
\captionof{figure}
{
More qualitative results compared to the state-of-the-art video inpainting methods FuseFormer~\cite{liu21fuseformer}, E$^2$FGVI~\cite{li22e2fgvi}, and FGT~\cite{zhang22flow}. \emph{Best viewed in color and by zooming in for all figures throughout the supplementary.}
}
\vspace*{0.2cm}
\label{fig:more_vi_compare}
